Greedy-Based Feature Selection for Efficient LiDAR SLAM

Modern LiDAR-SLAM (L-SLAM) systems have shown excellent results in large-scale, real-world scenarios. However, they commonly have a high latency due to the expensive data association and nonlinear optimization. This paper demonstrates that actively selecting a subset of features significantly improves both the accuracy and efficiency of an L-SLAM system. We formulate the feature selection as a combinatorial optimization problem under a cardinality constraint to preserve the information matrix's spectral attributes. The stochastic-greedy algorithm is applied to approximate the optimal results in real-time. To avoid ill-conditioned estimation, we also propose a general strategy to evaluate the environment's degeneracy and modify the feature number online. The proposed feature selector is integrated into a multi-LiDAR SLAM system. We validate this enhanced system with extensive experiments covering various scenarios on two sensor setups and computation platforms. We show that our approach exhibits low localization error and speedup compared to the state-of-the-art L-SLAM systems. To benefit the community, we have released the source code: https://ram-lab.com/file/site/m-loam.

==> exp-per-device.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Real-Time Performance on Embedded Computers}
\label{sec.exp-per-device}

==> problem.tex <==
%\begin{figure}
%	\centering
%	\includegraphics[width=0.47\textwidth]{figure/mlod_exp1-crop.pdf}
%	\caption{The propagated mean and covariance (shown as a one-standard-deviation ellipse) of a point over different $\alpha$ after transforming it into the base frame. We can see that (1) the variance becomes larger when $\alpha$ increases 1. $\alpha$ more covariance; 2. $\alpha$ has large variance.}       
%	\label{fig.problem_propagated_covariance}     
%	%\vspace{-0.5cm}    
%\end{figure}


%\begin{table}[]
%	\centering
%	\caption{Nomenclature of Section \ref{sec.problem}.}
%	\renewcommand\arraystretch{1.1}
%	%	\renewcommand\tabcolsep{3pt}        
%	\begin{tabular}{cc}
%		\hline
%		\toprule[0.03cm]
%		Notation & Explanation
%		\hline
%		\toprule[0.03cm]
%		$\{\}^{b}, \{\}^{l^{i}}$ & The frame of the based sensor and the $i^{th}$ LiDAR. We use $\{\}^{b}$ to represent $\{\}^{l^{1}}$.\\
%		\hline
%		\toprule[0.03cm]
%	\end{tabular}
%	\label{tab.lyft_acc_val}
%\end{table}

\begin{table}[]
	\centering
	\caption{Nomenclature}
	\renewcommand\arraystretch{1.1}
	%	\renewcommand\tabcolsep{3pt}   	
	\begin{tabularx}{0.47\textwidth}{cX}
		\hline
		\toprule[0.03cm]
		Notation & Explanation \\ 
		\hline
		\toprule[0.01cm]
		$\{\}^{b}, \{\}^{l^{i}}$ & Frame of the base and the $i^{th}$ LiDAR.\\
		$\mathcal{P}^{l^{i}}$ & Raw point cloud captured by the $i^{th}$ LiDAR.\\	
		$\mathcal{B}$ & Set of estimated 3D bounding boxes.\\		
%		$\mathcal{P}_{m}$ & The merged point cloud of all $\mathcal{P}^{l^{i}}$.\\				
		$\mathbf{T}$ & Transformation matrix in the \textit{Lie group} $SE(3)$.\\		
		$\mathbf{R}$ & Rotation matrix in the \textit{Lie group} $SO(3)$.\\				
		$\mathbf{t}$ & Translation vector in $\mathbb{R}^{3}$.\\						
		$\bm{\Theta}$ & Measurement and extrinsic uncertainty prior.\\
		$\bm{\Xi}$ & Associated covariance of each point.\\	
		$\alpha$ & Scaling parameter of $\bm{\Theta}$.\\
		\hline
		\toprule[0.03cm]		
	\end{tabularx}
	\label{tab.nomenclature}
	% \vspace{-0.3cm}
\end{table}



\section{Notations and Problem Statement}
\label{sec.notations_and_problem_statement}
% The nomenclature is shown in Tab. \ref{tab.nomenclature}.
% The transformation from $\{\}^{b}$ to $\{\}^{l^{i}}$ is denoted by $\mathbf{T}^{b}_{{l}^{i}}$. 
% Our perception system consists of multiple LiDARs, and the frame of the primary LiDAR, i.e. $l^{1}$, is considered as the base sensor.
% %Other LiDARs can be calibrated with the base sensor using the iterative closest point (ICP) technique \cite{pomerleau2013comparing}.
% Extrinsics describe the relative transformation from the base frame to other frames of auxiliary LiDARs. 
% With the extrinsics, all measurements or features from different LiDARs are transformed into the base frame for data fusion. 
% LiDARs are assumed to be synchronized, meaning that multiple point clouds are perceived at the same time.

The nomenclature is shown in Tab. \ref{tab.nomenclature}.
The transformation from $\{\}^{b}$ to $\{\}^{l^{i}}$ is denoted by $\mathbf{T}^{b}_{{l}^{i}}$. 
Our perception system consists of one primary LiDAR which is denoted by $l^{1}$ and multiple auxiliary LiDARs.
The primary LiDAR defines the base frame and the auxiliary LiDAR provides the additional field of view (FOV) and measurements to alleviate the occlusion problem and the sparsity drawback of the primary LiDAR.
Extrinsics describe the relative transformation from the base frame to other frames of auxiliary LiDARs. 
With the extrinsics, all measurements or features from different LiDARs are transformed into the base frame for data fusion. 
LiDARs are assumed to be synchronized, meaning that multiple point clouds are perceived at the same time.

In this paper, we focus on 3D object detection with a multi-LiDAR system. 
The extrinsic perturbation is also considered, which indicates the small but unexpected change on transformation from the base frame to other frames over time.
Our goal is to estimate a series of 3D bounding boxes covering objects of predefined classes.
Each bounding box $\mathbf{b}\in\mathcal{B}$ is parameterized as $[c, x,y,z,w,l,h,\gamma]$, $c$ is the class of a bounding box, $[x,y,z]$ denotes a box's bottom center, 
$[w,h,l]$ represent the sizes along the $x\textendash$, $y\textendash$, 
and $z\textendash$ axes respectively,
as well as $\gamma$ for the rotation of the 3D bounding box along the $z\textendash$ axis in the range of $(0, \pi]$.

%\sout{
%In the multi-LiDAR 3D object detection problem,
%the input is a set of point clouds captured by different LiDARs synchronously
%$\{P_i^{F_i}, i=1, ..., M\}$, where $M$ are the number of LiDARs.
%The goal is to find a set of 3D bounding boxes covering the object of pre-defined classes as its single-LiDAR counterpart.
%A set of 3D bounding boxes is parameterized as $B^{F_I} = \{b_i^{F_I}=[cls, x,y,z,w,l,h,\theta]| i=1,...,m\}$
%where $cls$ is the class of the bounding box, 
%and $[x,y,z]^{T}$ is the bottom center of the 3D bounding box,
%as well as $[w,h,l]$ is the size of the 3D bounding box along the x,y,z-axises respectively 
%(x and y axises define the ground plane in the right-handed coordinate system).
%$\theta$ is the rotation of the 3D bounding box along the z-axis in range of $(0, \pi]$.
%% The problem definition of multi-LiDAR 3D object detection is almost same to the single-LiDAR counterpart,
%% but the $T_{Ti}$ is not a perfect transformation matrix.
%}

